Fidelity-Imposed Displacement Editing for the Learn2Reg 2024 SHG-BF Challenge

Co-examination of second-harmonic generation (SHG) and bright-field (BF) microscopy enables the differentiation of tissue components and collagen fibers, aiding the analysis of human breast and pancreatic cancer tissues. However, large discrepancies between SHG and BF images pose challenges for current learning-based registration models in aligning SHG to BF. In this paper, we propose a novel multi-modal registration framework that employs fidelity-imposed displacement editing to address these challenges. The framework integrates batch-wise contrastive learning, feature-based pre-alignment, and instance-level optimization. Experimental results from the Learn2Reg COMULISglobe SHG-BF Challenge validate the effectiveness of our method, securing the 1st place on the online leaderboard.

==> docs/arxiv.tex <==
% In multimodal image registration, we observed significant structural dissimilarity between the fixed and moving images, with very little apparent correlation, as shown in Fig.~\ref{fig:quali}. To address this challenge, it is crucial to map the images from different modalities into a common latent space \(F_i\). By obtaining such a shared representation, the registration problem can be effectively simplified to monomodal registration, where established techniques are more readily applicable.

% Our prealignment model is inspired by the architecture of CoMIR \cite{pielawski2020comir} but incorporates two significant modifications to enhance performance. First, we replace the original noise-contrastive estimation (InfoNCE) loss with our specially designed batch-wise contrastive estimation (B-NCE) loss, tailored specifically for this task. Second, instead of employing classical feature-based registration methods like SIFT used in the original work, we adopt XFeat—a learning-based method—to achieve better registration accuracy. 

% We train the contrastive representation learning network jointly with the matching network in an end-to-end manner. From the trained network, we extract a prealigned affine transformation matrix \(\Phi_1(I_A, I_B)\), which serves as an initial alignment between the fixed and moving images.

% Similar to CoMIR, we utilize two identical Dense Tiramisu networks $D_{\theta_i}:\mathbb{R}^{2 \times \mathcal{C}} \rightarrow \mathbb{R}^2$, where $\mathcal{C}$ represent the channel dimension and $\theta$ represent the network parameters, to extract dense representations from the fixed and moving images, denoted as \(C_A=D_{\theta_1}(I_A)\) and \(C_B=D_{\theta_2}(I_B)\), respectively. To ensure that the learned common-space representations are content-informative and equivariant to rotations and translations, we train the network using our novel B-NCE loss within a contrastive learning framework. The main idea behind B-NCE is to formulate the loss criterion as a lower bound on the mutual information between different modalities, thereby encouraging the network to capture shared information across them.

% \noindent \textbf{B-NCE.} In our batch-wise Noise Contrastive Estimation (NCE) implementation, we begin by extracting small patches from the feature maps \(C_A\) and \(C_B\) of the fixed and moving images. We set the patch size to \(p \times p\), which results in \(N\) patches for each feature map, denoted as \((X_i, Y_i) \in \mathbb{R}^{N \times H \times W}\). We employ two different sampling methods, resulting in two groups of patch pairs. These patches are sampled to create overlapping regions that capture localized features, and are subsequently reshaped and processed through average pooling \(\mathcal{A}: \mathbb{R}^{ H \times W} \rightarrow \mathbb{R}^{h \times w}\), where \(h,w\) is the new dimension of the downsampled patches, reducing the spatial dimensions and creating $\mathbf{x}_i^k, \mathbf{y}_i^k\ \in \mathbb{R}^{1 \times h \times w}$.

% Traditional methods compute the similarity matrix across different batch samples, treating positive pairs as samples from the same batch locations. In contrast, we focus on enhancing position-level similarities for the same positions across the batch dimension. To achieve this, we stack all small batches along the batch dimension, resulting in tensors \(\mathbf{X}, \mathbf{Y} \in \mathbb{R}^{N \times h \times w}\), where \(N\) is the batch size and \(h \times w\) are the spatial dimensions. For each spatial position \((i, j) \in \mathbb{R}^{h \times w}\), we extract vectors \(\mathbf{X}_{i,j} \in \mathbb{R}^{N}\) that contain information from all batch samples at that specific position. Each position in \(\mathbf{X}\) and \(\mathbf{Y}\) thus aggregates data across all batches.

% We compute the similarity between \(\mathbf{X}_{i,j}\) and all other positions in both \(\mathbf{X}\) and \(\mathbf{Y}\) using the following formula:
% \[S(\mathbf{X}_{i,j}, (\mathbf{X}, \mathbf{Y})) = -\frac{1}{\tau} \left\| \mathbf{X}_{i,j} - \bigcup_{i,j}^{h,w} (\mathbf{X}, \mathbf{Y}) \right\|_1\] 
% where $S(\mathbf{Y}_{i,j}, (\mathbf{X}, \mathbf{Y})) \in \mathbb{R}^{(h \times w) \times [2 \times (h \times w)]}$ \(\tau\) is the temperature parameter. Similarly, we compute \(S(\mathbf{Y}_{i,j}, (\mathbf{X}, \mathbf{Y})) \in \mathbb{R}^{(h \times w) \times [2 \times (h \times w)]}\) in the same manner.

% The resultant downsampled patches from the two modalities are then concatenated as \(\mathcal{P}_1 = [\mathbf{x_1}, \mathbf{y_1}] \in \mathbb{R}^{2N \times c}\) and \(\mathcal{P}_2 = [\mathbf{y_2}, \mathbf{x_2}]\). We then compute the similarity between \(\mathbf{x_1}\) and all patches in \(\mathcal{P}_1\):$ S(\mathbf{x_1}, \mathcal{P}_1) = -\frac{1}{\tau} \lVert \mathbf{x_1} - \mathcal{P}_1 \rVert_1 \in \mathbb{R}^{N \times 2N}$ where \(\tau\) is the temperature parameter. Similarly, we compute \(S(\mathbf{y_2}, \mathcal{P}_2)\).

% The positive similarities \(S_{pos}\) are extracted from the corresponding patches between both modalities: $S_{pos} = S(\mathbf{X}_{i,j}, \mathbf{Y}_{i,j})$
% The negative similarities \(S_{neg}\) are defined as:
% $S{neg} = \sum_{i, j, k}^{2(h \times w) - 1} S(\mathbf{X}_{i,k}, \mathbf{Y}_{i,j}) - S(\mathbf{X}_{i,k}, \mathbf{X}_{i,k})$.

% We use a contrastive loss function inspired by InfoNCE. For each positive pair, the loss can be expressed as:
% \begin{equation}
%     \mathcal{L}_{\text{NCE}} = -\frac{1}{h \times w} \sum_{i, j}^{h, w} \log \frac{\exp\left(\frac{S_{pos}^{i,j}}{\tau}\right)}{\exp\left(\frac{S_{pos}^{i,j}}{\tau}\right) + \sum_{k \neq j} \exp\left(\frac{S_{neg}^{i,k}}{\tau}\right)}
% \end{equation}
% where \(S_{pos}^i\) is the similarity of the \(i\)-th positive pair, and \(D_{neg}\) is the set of all negative pairs. Minimizing this loss approximately maximizes a lower bound on the mutual information (MI) between the different modalities.

% The final NCE loss is a combination of the losses computed for both directions (\(\mathbf{X \rightarrow Y}\) and \(\mathbf{Y \rightarrow X}\)):
% \begin{equation}
%     \mathcal{L}_{\text{B-NCE}} = \mathcal{L}_{\text{NCE}}(\mathbf{X}, \mathbf{Y}) + \mathcal{L}_{\text{NCE}}(\mathbf{Y}, \mathbf{X})
% \end{equation}


%% trim a little bit
% \noindent \textbf{XFeat.} We adapt the XFeat \cite{siebert2021fast} feature detection and matching given the monomodality representation learnt above. As XFeat was previsouly designed for RGB images, we replicate the learnt representations to $\mathbf{x'}, \mathbf{y'} \in \mathbb{R}^{3 \times H \times W}$. We apply two distinct geometric augmentations $H_1$ as basic affine geometric transformation while  $H_2$ is treat as complex augmentation using Thin Plate Spline (TPS) deformations. The XFeat model is then employed to extract dense matching pairs $N$ are extracted at a coarse scale of $1/8$. We obtained $M$ pairs of matching keypoints coordinates $p_x, p_y$ and their corresponding dense features $m_i \in \mathcal{R}^{M \times 64}, i\in[x,y]$ and reliability heatmaps $h_i \in \mathcal{R}^{M \times 1}, i\in[x,y]$. We can determine the postive matching pairs based on the homographies, which allow us to determine the matching locations. We follow the same setting to compute the consistency loss for cooridnates and feature maps denoted as $L_{XFeat}$

% Thus the final training loss is summarized as $L = L_{B-NCE} + L_{XFeat}$

%\textbf{Dual Softmax Loss:} Measures the similarity between the dense features $m_1$ and $m_2$ by computing a temperature-scaled dot product and applying the softmax function. It calculates the negative log-likelihood of matching pairs in both directions, providing confidence scores for the matches. \textbf{Coordinate Classification Loss:} Optimizes fine coordinate classification by comparing predicted coordinates $p_i$ with the true offsets of detected keypoints within grid cells. The loss is weighted by confidence scores to emphasize reliable matches and includes accuracy measurement of coordinate predictions. \textbf{Keypoint Loss:} Evaluates the difference between predicted heatmaps $h_i$ and target confidence values for keypoints $p_i$ using the L1 loss, penalizing discrepancies in keypoint localization to ensure accurate keypoint predictions.


% This step normalizes and aligns the images by stretching them into a common space, accommodating significant variations between them. The features, denoted as  for SHG images and $F_y$ for BF images, are extracted using a pre-trained Tiramisu network and then passed to the initial alignment stage.

% The training of the Tiramisu network follows prior work COMIR \cite{pielawski2020comir} in the context of contrastive learning with certain modifications.
% To enhance robustness, we introduce a batch-based Noise Contrastive Estimation (NCE) loss \cite{gutmann2010noise}. Small patches from the feature maps are sampled using two different backbone models for each modality, forming $P_{x1}, P_{x2}$ and $P_{y1}, P_{y_2}$. These paired patches are used for bidirectional contrastive loss, $P_{x_1} \rightarrow P_{y1}$ and $P_{x_2} \leftarrow P_{y2}$
% The NCE loss compares stacks of features across the same spatial position in different patches, leveraging batch-wise context to improve alignment accuracy. The extracted patches from $P_x, P_y$ are concatenated along the patch dimension, creating a combined set of patches. Similarities between patches are calculated using a critic function (L1 distance), scaled by a temperature parameter $\tau=0.5$ to control the sharpness of the distribution. Positive similarity scores are obtained by comparing each patch in $P_{anchor}^+$ with its corresponding patch in $P_{anchor}^-$ while negative similarity scores are computed by comparing the patch with all other patches in the combined set, excluding self-similarity. The final NCE loss is computed by taking the difference between the negative log-likelihood of the positive scores and the log-sum-exp of the negative scores. This approach ensures robust and consistent feature matching by considering spatial relationships within a batch.

